Use Cases, Metrics, and Challenges of Nomadic Non-Public Networks for the 6G Standardization

Wireless communication is evolving with the adoption of dynamic and self-organizing networks. They are expected to play a crucial role in shaping sixth-generation (6G) systems and the ongoing standardization process. The concept of non-public networks (NPNs) introduced in fifth-generation (5G) will be enhanced by nomadic non-public networks (NNPNs), extending mobility and adaptability beyond fixed locations. These networks help overcome the limitations of traditional static infrastructures, making them applicable to areas such as emergency response, transportation, agriculture, and others. This paper examines the transition from NPNs to NNPNs, highlighting key technical aspects such as network architecture, dynamic resource allocation, and wireless backhauling. Several use cases illustrate how NNPNs improve connectivity in environments where traditional networks are limited. Additionally, the study defines Key Performance Indicators (KPIs) to evaluate NNPN applications and establishes a framework for categorizing them based on mobility and operational requirements. Despite their advantages, NNPNs introduce architectural, regulatory, and security challenges such as new approaches for handovers, spectrum policies or cross-border functionality, and trust mechanisms to maintain reliable operations. By identifying use cases, defining evaluation criteria, and addressing technical and regulatory challenges, this paper provides insights into integrating NNPNs into future 6G networks. These findings contribute to ongoing standardization efforts and emphasize the need for adaptable policies and network architectures to maximize the benefits of NNPNs in next-generation communication systems.

==> 0mainDenKr.tex <==
% !TEX root = 1main.tex
%%###########################################################%%
%%        vvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvv        %%
%%-----------------------------------------------------------%%
%  Author of Boilerplate / Template / LaTeX-Document Skeleton:
%      - Dennis Krummacker
%  Created:
%      2016
%  Last Update:
%      2024-01
%  Latest Compiler Tool-Chain to be compatible (recommended to run with):
%      TeXLive-2023
%  Compiler to use:
%      pdfLaTeX
%  Recommended Arguments:
%      -synctex=1 -interaction=nonstopmode --shell-escape
%%------------------------------------------------------------%%
%%        ^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^        %%
%%============================================================%%
%
%
%
%==================================================================================
% ----  Cmd-Line Arguments
% ----    Yes, ehem, I created something that behaves like Cmd-Line Arguments...
% ----    You may safely ignore this. It shouldn't interfer with cases, where they are not provided.
%----------------------------------------------------------------------------------
% TeX booleans start out as false.
\newif\ifMyScreenOutput%
% What follows uses LaTeX3 syntax.
\ExplSyntaxOn%
% LaTeX3 bools start out as false too.
\bool_new:N \g_DenKrCmdLineArgs_screenOutput_bool
% Our LaTeX3 error message(s) for the option list parser (l10n-ready)
\msg_new:nnnn {DenKrCmdLineArgs} {unknown-choice-for-option}%
  {%
    Invalid~value~for~option~\exp_not:n {'#1'}:~\exp_not:n {'#3'}~%
    (valid~choices~are~\exp_not:n {#2})%
  }%
  {You~may~optionally~put~a~more~verbose~message~here.}%
% Option definitions for our pseudo-package 'DenKrCmdLineArgs' (this document). See l3keys in interface3.pdf as found at [1].
%   [1] https://ctan.org/pkg/l3kernel
\keys_define:nn {DenKrCmdLineArgs}%
  {%
    % First accepted key: 'outputType'. It takes an optional value among a fixed, limited number of choices, as defined next.
    outputType .choice:,%
    outputType / paper .code:n = {     % The first such value is 'paper'.
      \bool_gset_false:N \g_DenKrCmdLineArgs_screenOutput_bool},%
    outputType / screen .code:n = {    % The second one is 'screen'.
      \bool_gset_true:N \g_DenKrCmdLineArgs_screenOutput_bool},%
    outputType .initial:n = {paper}, % Default is 'paper'
    outputType / unknown .code:n = {   % Run this when passed an invalid value.
      \msg_error:nnxxx {DenKrCmdLineArgs} {unknown-choice-for-option}%
        {outputType}                 % name of the choice key
        {'paper'~and~'screen'}       % valid choices
        {\exp_not:n {#1}}            % invalid choice given
    },%
    % Second accepted key: 'srcSubDir'. Whether the Project's source is put into a sub-directory.
    srcSubDir .tl_set:N = \l_DenKrCmdLineArgs_srcSubDir_tl,%
    srcSubDir .initial:n = {}, % the default is empty
    % Used when the key is passed with no value ('fullScreen' as opposed to 'fullScreen=something'
    srcSubDir .default:n = {}%
  }%
% The option values may be set from the command line by means of the \DenKrCmdLineArgs macro, which may be defined this way before \input{}ing this file. For the precise option syntax, see l3keys in interface3.pdf[1].
%   \newcommand{\MyDocParams}{
%       outputType=screen,
%       srcSubDir="src"
%   }
% Since we already set defaults above with \keys_define:nn, no need to set any here. But Provide it, so that no error is thrown in absence.
\providecommand{\DenKrCmdLineArgs}{}%
% This is where keys are set from the point of view of l3keys, and the action associated with each option set is carried out.
% In order to obtain the option list, we expand once ('o') the second argument of \keys_set:no, namely the \DenKrCmdLineArgs token.
\keys_set:no {DenKrCmdLineArgs} {\DenKrCmdLineArgs}%
% Finally, convert the LaTeX3 booleans to \ifFooBar TeX conditionals. This is more or less needed, because control sequences such as \g_DenKrCmdLineArgs_screenOutput_bool will be difficult to enter in the main part of the document without using \ExplSyntaxOn ... \ExplSyntaxOff every time, which would be quite ugly.
% Of course, instead of the TeX conditionals, one could use booleans from the 'ifthen' or 'etoolbox' packages.
\bool_if:NT \g_DenKrCmdLineArgs_screenOutput_bool%
  {\MyScreenOutputtrue}%
\tl_set_eq:NN \DenKrNestedSrcDirArg \l_DenKrCmdLineArgs_srcSubDir_tl%
%
\ExplSyntaxOff%
\providecommand{\DenKrNestedSrcDirArg}{default}%
\typeout{»DenKr:  Compiling from nested Src-Dir: "\DenKrNestedSrcDirArg"}%
%
%
%
%==================================================================================
% ----  Custom-Generated-File Reading
% ----    With my latexmkrc for local compilation, a Custom-File is generated during Compilation and put to the tmp-dir.
%----------------------------------------------------------------------------------
% A Macro for this is defined in "0organization/1main/2includes/setup/tex_primitive_cmd.exe", but this is not yet included here.
%   Nothing like that is currently required here.
%
%
%
%
%
% When wrapping the entire Project into Sub-Directory, either set a latexmkrc file to pass this as Argument.
%   Or directly set \DenKrNestedSrcDir directly below this Comment
%==================================================================================
% ----  Setup
%----------------------------------------------------------------------------------
\newcommand{\DenKrSetupFilesSubDirPrefix}{0DenKrFrame/}% {./}  \DenKrNestedSrcDir
\newcommand{\DenKrSubDirPrefix}{\DenKrSetupFilesSubDirPrefix}%
%
\newcommand{\DenKrProjectSetupFILE}{2ProjectSetup}%
\input{"\DenKrSetupFilesSubDirPrefix\DenKrProjectSetupFILE".tex}%
%
%
%
%
%
%==================================================================================
% ----  Inclusions
%----------------------------------------------------------------------------------
\input{"\DenKrLayoutMainRootDir/preamble".tex}%
\input{"\DenKrLayoutMainRootDir/makros".tex}%
\input{"\DenKrLayoutMainRootDir/makros_typografie".tex}%
\input{"\DenKrLayoutMainRootDir/3settings/settings_basic".tex}%
\input{"\DenKrLayoutMainRootDir/settings_perDoc".tex}%
%
%   \input{"\DenKrLayoutBaseRootDir/standalone_constituent/macro_exclusionMux".tex}% -->
\newcommand{\onlyinsubfile}[1]{}%
\newcommand{\notinsubfile}[1]{#1}%
\newcommand{\onlyinmainfile}[1]{\notinsubfile{#1}}%
%
\input{"\DenKrSupplyRootDir/TitlePage_Data".tex}%
%
%
%
\usepackage{verbatim}
%
%
%______________________________________________________________
%\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\......
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%#############################################################################%%
\begin{document}%%#############################################################%%
%%#############################################################################%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%////////////////////////////////////////////////////////////////////´´´´´´
%''''''''''''''''''''''''''''''''''''''''''''''''''''''''''''''
%

\input{"\DenKrLayoutRootDir/TitlePage".tex}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%#############################################################################%%
%VVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVV%
%
%
%
\newcommand{\DenKrDispositionFILE}{3Disposition}%
\input{"\DenKrSetupFilesSubDirPrefix\DenKrDispositionFILE".tex}%
%
%
%
%
\input{"\DenKrLayoutRootDir/postamble".tex}%
%
\end{document}%
%

==> 2_abstract.tex <==
% !TEX root = ../../1main.tex
%
% \textcolor{green}{Look into\nl \enquote{\DenKrSegmentationSubDir/100\_abstract.tex}}
%
% Abstract of not more than 250 words. (Preferably not less than 150 words.)
%======================================
%English Abstract
Wireless communication is evolving with the adoption of dynamic and self-organizing networks. They are expected to play a crucial role in shaping \gls{6g} systems and the ongoing standardization process. The concept of \glspl{npn} introduced in \gls{5g} will be enhanced by \glspl{nnpn}, extending mobility and adaptability beyond fixed locations. These networks help overcome the limitations of traditional static infrastructures, making them applicable to areas such as emergency response, transportation, agriculture, and others. This paper examines the transition from \glspl{npn} to \glspl{nnpn}, highlighting key technical aspects such as network architecture, dynamic resource allocation, and wireless backhauling. Several use cases illustrate how \glspl{nnpn} improve connectivity in environments where traditional networks are limited. Additionally, the study defines \glspl{kpi} to evaluate \gls{nnpn} applications and establishes a framework for categorizing them based on mobility and operational requirements. Despite their advantages, \glspl{nnpn} introduce architectural, regulatory, and security challenges such as new approaches for handovers, spectrum policies or cross-border functionality, and trust mechanisms to maintain reliable operations.
%Despite their advantages, \glspl{nnpn} introduce architectural and regulatory challenges. Their mobility contrasts with existing network models, requiring new approaches for handovers, interference management, and spectrum allocation. Security concerns also arise, necessitating enhanced authentication and trust mechanisms to maintain reliable operations. Furthermore, regulatory issues, particularly regarding spectrum policies and cross-border functionality, complicate widespread adoption and standardization.
By identifying use cases, defining evaluation criteria, and addressing technical and regulatory challenges, this paper provides insights into integrating \glspl{nnpn} into future \gls{6g} networks. These findings contribute to ongoing standardization efforts and emphasize the need for adaptable policies and network architectures to maximize the benefits of \glspl{nnpn} in next-generation communication systems.





